PaliGemma: A versatile 3B VLM for transfer

PaliGemma is an open Vision-Language Model (VLM) that is based on the SigLIP-So400m vision encoder and the Gemma-2B language model. It is trained to be a versatile and broadly knowledgeable base model that is effective to transfer. It achieves strong performance on a wide variety of open-world tasks. We evaluate PaliGemma on almost 40 diverse tasks including standard VLM benchmarks, but also more specialized tasks such as remote-sensing and segmentation.

==> tables/results_refcocoseg.tex <==
\begin{table*}[ht]
\setlength{\tabcolsep}{0pt}
\setlength{\extrarowheight}{5pt}
\renewcommand{\arraystretch}{0.75}
\newcolumntype{C}{>{\centering\arraybackslash}X}
\newcolumntype{R}{>{\raggedleft\arraybackslash}X}
\centering \scriptsize
\caption{mIoU on RefCOCO segmentation results.}
\label{tbl:main_refseg}
\vspace{-2mm}
\begin{tabularx}{\linewidth}{>{\hsize=1.4\hsize}X>{\hsize=.6\hsize}X>{\hsize=.8\hsize}X>{\hsize=.8\hsize}X>{\hsize=.8\hsize}X>{\hsize=.8\hsize}X>{\hsize=.8\hsize}X>{\hsize=.8\hsize}X>{\hsize=.8\hsize}X}
 \toprule[1pt]

\multirow{2}{*}{\textbf{MODEL}} & \multicolumn{3}{c}{RefCOCO} & \multicolumn{3}{c}{\hspace{5pt} RefCOCO+} & \multicolumn{2}{c}{RefCOCOg} \\
\cmidrule(r{15pt}){2-4} \cmidrule(l{0pt}r{16pt}){5-7} \cmidrule(l{0pt}r{11pt}){8-9}
& val & testA & testB & val & testA & testB & val-u & test-u \\
    \midrule

pt\_224 & 73.40 & 75.73 & 70.67 & 68.32 & 71.86 & 64.52 & 67.65 & 68.24 \\
pt\_448 & 75.57 & 77.94 & 72.36 & 69.76 & 74.24 & 64.55 & 70.17 & 71.04 \\
pt\_896 & 76.94 & 78.67 & 73.94 & 72.18 & 76.06 & 66.91 & 72.22 & 72.72 \\

\bottomrule
\end{tabularx}
\vspace{-2mm}
\end{table*}
